3D Spatial Pattern Matching

Spatial pattern matching is the process of matching query entities and constraints with database entities and relations. It has many applications, including similar region search, housing market search, landmark search, and road network matching. To our knowledge, all existing spatial pattern matching approaches frame the problem in a 2 dimensional space, where entities lie in a cartesian plane and relationships defined between them are contained in 2 dimensions. However, this problem framing has significant limitations when searching for real world entities that have height in addition to position. To address this limitation, we extend spatial pattern matching to 3 dimensions and provide a generalized definition of the problem. We describe a subgraph matching algorithm capable of resolving 3D spatial patterns over distance relations and release two 3D spatial pattern matching datasets, one synthetic and one containing real 3D building data from the city of Hamburg, Germany. We test our subgraph matching algorithm on both datasets and present results as a baseline for future methods to build upon.

==> sections/NA_Dataset_Table.tex <==
\begingroup
\renewcommand{\arraystretch}{1.03}
\begin{table}[ht]
    \small
    \centering
    \begin{tabular}{cclll}
    \hline
        \textbf{Dataset} & \textbf{Geographic Region} & \textbf{$|D|$} & \textbf{$U$}\\
        \hline
        Synthetic  & - & ? & ? \\
        ..         & ? & ? & ? \\
    \hline
    \end{tabular}
    \caption{Summary of datasets. $|D|$ is the number of entities. $U$ is the number of unique entity classes.}
    \label{tab:datasets}
\end{table}
\endgroup
